SynFuzz: Leveraging Fuzzing of Netlist to Detect Synthesis Bugs

In the evolving landscape of integrated circuit (IC) design, the increasing complexity of modern processors and intellectual property (IP) cores has introduced new challenges in ensuring design correctness and security. The recent advancements in hardware fuzzing techniques have shown their efficacy in detecting hardware bugs and vulnerabilities at the RTL abstraction level of hardware. However, they suffer from several limitations, including an inability to address vulnerabilities introduced during synthesis and gate-level transformations. These methods often fail to detect issues arising from library adversaries, where compromised or malicious library components can introduce backdoors or unintended behaviors into the design. In this paper, we present a novel hardware fuzzer, SynFuzz, designed to overcome the limitations of existing hardware fuzzing frameworks. SynFuzz focuses on fuzzing hardware at the gate-level netlist to identify synthesis bugs and vulnerabilities that arise during the transition from RTL to the gate-level. We analyze the intrinsic hardware behaviors using coverage metrics specifically tailored for the gate-level. Furthermore, SynFuzz implements differential fuzzing to uncover bugs associated with EDA libraries. We evaluated SynFuzz on popular open-source processors and IP designs, successfully identifying 7 new synthesis bugs. Additionally, by exploiting the optimization settings of EDA tools, we performed a compromised library mapping attack (CLiMA), creating a malicious version of hardware designs that remains undetectable by traditional verification methods. We also demonstrate how SynFuzz overcomes the limitations of the industry-standard formal verification tool, Cadence Conformal, providing a more robust and comprehensive approach to hardware verification.

==> ML_HS.tex <==

\section{ML for Hardware Verification}
\label{ml_hs}



It is estimated that verification engineers spend up to 70\% of their time on the verification phase in the modern IC design cycle \cite{vlsibook}. Machine Learning (ML) facilitates learning through training on data and evolutionary improvements, making it effective in handling both familiar and unseen data patterns. To reduce the manual intervention required from verification engineers, recent research trends focus on deploying ML techniques to automate various aspects of the verification process. By leveraging ML, tasks such as test case generation, bug detection, and coverage analysis can be automated, significantly reducing the time and effort required for verification while enhancing accuracy and coverage \cite{Selvakkumaran'03,Lee'08,Hamilton'17,Ying'18}. While applying Machine Learning (ML) to hardware verification, several key requirements must be met for effective implementation: \textbf{\textit{1) Definition of Problem Statement 2) Selection of Appropriate Hardware Abstraction Level 3) Selection of Processes to Automate 4) Generation of Unbiased, Realistic, and Comprehensive Data. }} In recent years there has been an exponential increase in the number of hardware verification works but not limited to the detection of trojans, securing designs against reverse engineering through ML, test case generation, side-channel analysis, and many more \cite{Cai'16,Ma'19,Haaswijk'18,Xie'18,Chan'16}. One such ML technique is the  Graph Learning algorithm, which is used in a diverse range of hardware security applications \cite{Selvakkumaran'03,Lee'08,Hamilton'17,Ying'18}.


\vspace{-1 em}

\subsection{Graph Learning for IC Security} \label{gleda}
Graph Neural Networks (GNNs) have gained significant attention due to their superior performance in graph-based learning tasks, as highlighted in several studies \cite{Cai'18,Grover'16,Kahng'10,Yu'11,Cheng'95,Rozhin'21}. The success of GNNs in EDA is largely attributed to the fact that Boolean circuits can be naturally represented as graphs. A key factor driving the adoption of graph learning techniques \cite{Hamilton'17,Cao'15} over other methods is their ability to generalize, handle diverse topologies, scale efficiently, and be structurally aware, which serves as a \textit{primary motivation for us to choose graph learning in our work, GLFuzz}. In contrast, traditional machine learning approaches, such as Deep Neural Networks (DNNs) and Convolutional Neural Networks (CNNs), have been widely applied across various EDA applications \cite{Cai'16,Chan'16,Chan'17,Jeong'10}, however, they require grid-based data or design representations  \cite{Hamilton'17,Cao'15}, limiting their use to specific topologies. Researchers have successfully applied GNNs to a range of electronic design automation (EDA) challenges, including detecting hardware Trojans (HTs) \cite{Yasaei2021GNN4TJGN,Yu2021HW2VECAG}, identifying IP piracy \cite{Baehr2019MachineLA}, reverse engineering gate-level netlists \cite{gnnre} to name a few.


